Applications of Deep Learning for Ill-Posed Inverse Problems Within Optical Tomography

Increasingly in medical imaging has emerged an issue surrounding the reconstruction of noisy images from raw measurement data. Where the forward problem is the generation of raw measurement data from a ground truth image, the inverse problem is the reconstruction of those images from the measurement data. In most cases with medical imaging, classical inverse Radon transforms, such as an inverse Fourier transform for MRI, work well for recovering clean images from the measured data. Unfortunately in the case of X-Ray CT, where undersampled data is very common, more than this is needed to resolve faithful and usable images. In this paper, we explore the history of classical methods for solving the inverse problem for X-Ray CT, followed by an analysis of the state of the art methods that utilize supervised deep learning. Finally, we will provide some possible avenues for research in the future.

==> __latexindent_temp.tex <==
Automatically generated by Mendeley Desktop 1.19.4
Any changes to this file will be lost if it is regenerated by Mendeley.

BibTeX export options can be customized via Preferences -> BibTeX in Mendeley Desktop

@article{wang2016perspective,
abstract = {The combination of tomographic imaging and deep learning, or machine learning in general, promises to empower not only image analysis but also image reconstruction. The latter aspect is considered in this perspective article with an emphasis on medical imaging to develop a new generation of image reconstruction theories and techniques. This direction might lead to intelligent utilization of domain knowledge from big data, innovative approaches for image reconstruction, and superior performance in clinical and preclinical applications. To realize the full impact of machine learning for tomographic imaging, major theoretical, technical and translational efforts are immediately needed.},
archivePrefix = {arXiv},
arxivId = {1609.04375},
author = {Wang, Ge},
doi = {10.1109/ACCESS.2016.2624938},
eprint = {1609.04375},
file = {:Users/ap/Downloads/07733110.pdf:pdf},
issn = {21693536},
journal = {IEEE Access},
keywords = {Tomographic imaging,big data,data acquisition,deep learning,image analysis,image reconstruction,machine learning,medical imaging},
pages = {8914--8924},
publisher = {IEEE},
title = {{A perspective on deep imaging}},
volume = {4},
year = {2016}
}
@article{Lunz2018,
abstract = {Inverse Problems in medical imaging and computer vision are traditionally solved using purely model-based methods. Among those variational regularization models are one of the most popular approaches. We propose a new framework for applying data-driven approaches to inverse problems, using a neural network as a regularization functional. The network learns to discriminate between the distribution of ground truth images and the distribution of unregularized reconstructions. Once trained, the network is applied to the inverse problem by solving the corresponding variational problem. Unlike other data-based approaches for inverse problems, the algorithm can be applied even if only unsupervised training data is available. Experiments demonstrate the potential of the framework for denoising on the BSDS dataset and for computed tomography reconstruction on the LIDC dataset.},
archivePrefix = {arXiv},
arxivId = {1805.11572},
author = {Lunz, Sebastian and {\"{O}}ktem, Ozan and Sch{\"{o}}nlieb, Carola Bibiane},
eprint = {1805.11572},
file = {:Users/ap/Downloads/1805.11572.pdf:pdf},
issn = {10495258},
journal = {Advances in Neural Information Processing Systems},
number = {NeurIPS},
pages = {8507--8516},
title = {{Adversarial regularizers in inverse problems}},
volume = {2018-Decem},
year = {2018}
}
@inproceedings{zhao2017few,
abstract = {To reduce patient's dose, few-view CT reconstruction promises to be a good attempt. The key to better reconstruction is the sparse view artifacts. In recent years, DL(deep learing) has attracted a lot of attention because its outstanding performance in image processing. We propose a deep learning method for few-view CT reconstuction. Our method directly learns an end-to-end mapping between the full-view/few-view reconstruction. The mapping is represented as a deep convolutional neural network (CNN) that takes the few-view reconstruction image as the input and outputs the full-view one. We further show that traditional Dictionary Learning based reconstruction methods can also be viewed as a deep convolutional network. But unlike traditional methods that handle each component separately, our method jointly optimizes all layers. Our deep CNN has a lightweight structure, yet demonstrates state-of-theart reconstruction quality, and achieves fast speed for practical on-line usage. We explore different network structures and parameter settings to achieve trade-offs between performance and speed.},
author = {Zhao, Ji and Chen, Zhiqiang and Zhang, Li and Jin, Xin},
booktitle = {2016 IEEE Nuclear Science Symposium, Medical Imaging Conference and Room-Temperature Semiconductor Detector Workshop, NSS/MIC/RTSD 2016},
doi = {10.1109/NSSMIC.2016.8069593},
isbn = {9781509016426},
issn = {null},
keywords = {CNN,Computed Tomography,Deep Learning,Few-view},
month = {oct},
pages = {1--4},
title = {{Few-view CT reconstruction method based on deep learning}},
volume = {2017-Janua},
year = {2017}
}
@article{Kang2018,
abstract = {Model-based iterative reconstruction algorithms for low-dose X-ray computed tomography (CT) are computationally expensive. To address this problem, we recently proposed a deep convolutional neural network (CNN) for low-dose X-ray CT and won the second place in 2016 AAPM Low-Dose CT Grand Challenge. However, some of the textures were not fully recovered. To address this problem, here we propose a novel framelet-based denoising algorithm using wavelet residual network which synergistically combines the expressive power of deep learning and the performance guarantee from the framelet-based denoising algorithms. The new algorithms were inspired by the recent interpretation of the deep CNN as a cascaded convolution framelet signal representation. Extensive experimental results confirm that the proposed networks have significantly improved performance and preserve the detail texture of the original images.},
archivePrefix = {arXiv},
arxivId = {1707.09938},
author = {Kang, Eunhee and Chang, Won and Yoo, Jaejun and Ye, Jong Chul},
doi = {10.1109/TMI.2018.2823756},
eprint = {1707.09938},
file = {:Users/ap/Downloads/1707.09938.pdf:pdf},
issn = {1558254X},
journal = {IEEE Transactions on Medical Imaging},
keywords = {Deep learning,convolution framelets,convolutional neural network (CNN),framelet denoising,low-dose CT},
number = {6},
pages = {1358--1369},
title = {{Deep Convolutional Framelet Denosing for Low-Dose CT via Wavelet Residual Network}},
volume = {37},
year = {2018}
}
@article{zhang2017beyond,
author = {Zhang, Kai and Zuo, Wangmeng and Chen, Yunjin and Meng, Deyu and Zhang, Lei},
file = {:Users/ap/Downloads/07839189.pdf:pdf},
journal = {IEEE Transactions on Image Processing},
number = {7},
pages = {3142--3155},
publisher = {IEEE},
title = {{Beyond a gaussian denoiser: Residual learning of deep cnn for image denoising}},
volume = {26},
year = {2017}
}
@article{adler2018learned,
author = {Adler, Jonas and {\"{O}}ktem, Ozan},
file = {:Users/ap/Downloads/1707.06474.pdf:pdf},
journal = {IEEE transactions on medical imaging},
number = {6},
pages = {1322--1332},
publisher = {IEEE},
title = {{Learned primal-dual reconstruction}},
volume = {37},
year = {2018}
}
@article{Putzky2017,
abstract = {Much of the recent research on solving iterative inference problems focuses on moving away from hand-chosen inference algorithms and towards learned inference. In the latter, the inference process is unrolled in time and interpreted as a recurrent neural network (RNN) which allows for joint learning of model and inference parameters with back-propagation through time. In this framework, the RNN architecture is directly derived from a hand-chosen inference algorithm, effectively limiting its capabilities. We propose a learning framework, called Recurrent Inference Machines (RIM), in which we turn algorithm construction the other way round: Given data and a task, train an RNN to learn an inference algorithm. Because RNNs are Turing complete [1, 2] they are capable to implement any inference algorithm. The framework allows for an abstraction which removes the need for domain knowledge. We demonstrate in several image restoration experiments that this abstraction is effective, allowing us to achieve state-of-the-art performance on image denoising and super-resolution tasks and superior across-task generalization.},
archivePrefix = {arXiv},
arxivId = {1706.04008},
author = {Putzky, Patrick and Welling, Max},
eprint = {1706.04008},
file = {:Users/ap/Downloads/1706.04008.pdf:pdf},
number = {Nips},
title = {{Recurrent Inference Machines for Solving Inverse Problems}},
url = {http://arxiv.org/abs/1706.04008},
year = {2017}
}
@article{Boink2018,
abstract = {We replace part of a model-based iterative algorithm with a convolutional neural network in order to improve the quality of tomography reconstructions. We analyse its robustness against uncertainties in the image and uncertainties in system settings. Results are presented for the application of photoacoustic tomography in a limited angle setup.},
author = {Boink, Yoeri E. and van Gils, Stephan A. and Manohar, Srirang and Brune, Christoph},
doi = {10.1002/pamm.201800222},
file = {:Users/ap/Downloads/pamm.201800222.pdf:pdf},
issn = {1617-7061},
journal = {Pamm},
number = {1},
pages = {10--11},
title = {{Sensitivity of a partially learned model‐based reconstruction algorithm}},
volume = {18},
year = {2018}
}
@article{Lecun2015,
abstract = {Deep learning allows computational models that are composed of multiple processing layers to learn representations of data with multiple levels of abstraction. These methods have dramatically improved the state-of-the-art in speech recognition, visual object recognition, object detection and many other domains such as drug discovery and genomics. Deep learning discovers intricate structure in large data sets by using the backpropagation algorithm to indicate how a machine should change its internal parameters that are used to compute the representation in each layer from the representation in the previous layer. Deep convolutional nets have brought about breakthroughs in processing images, video, speech and audio, whereas recurrent nets have shone light on sequential data such as text and speech.},
author = {Lecun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
doi = {10.1038/nature14539},
file = {:Users/ap/Downloads/DeepLearning{\_}LeCun.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7553},
pages = {436--444},
pmid = {26017442},
title = {{Deep learning}},
volume = {521},
year = {2015}
}
@article{jin2017deep,
author = {Jin, Kyong Hwan and McCann, Michael T and Froustey, Emmanuel and Unser, Michael},
file = {:Users/ap/Downloads/07949028.pdf:pdf},
journal = {IEEE Transactions on Image Processing},
keywords = {Denoiser},
mendeley-tags = {Denoiser},
number = {9},
pages = {4509--4522},
publisher = {IEEE},
title = {{Deep convolutional neural network for inverse problems in imaging}},
volume = {26},
year = {2017}
}
@article{arridge2019solving,
abstract = {Recent research in inverse problems seeks to develop a mathematically coherent foundation for combining data-driven models, and in particular those based on deep learning, with domain-specific knowledge contained in physical-analytical models. The focus is on solving ill-posed inverse problems that are at the core of many challenging applications in the natural sciences, medicine and life sciences, as well as in engineering and industrial applications. This survey paper aims to give an account of some of the main contributions in data-driven inverse problems.},
author = {Arridge, Simon and Maass, Peter and {\"{O}}ktem, Ozan and Sch{\"{o}}nlieb, Carola Bibiane},
doi = {10.1017/S0962492919000059},
file = {:Users/ap/Downloads/ArridgeMOC{\_}DLIP{\_}review{\_}ActaNumerica{\_}2019.pdf:pdf},
issn = {14740508},
journal = {Acta Numerica},
pages = {1--174},
publisher = {Cambridge University Press},
title = {{Solving inverse problems using data-driven models}},
volume = {28},
year = {2019}
}
@article{Arridge1997,
abstract = {Optical tomography is a new medical imaging modality that is at the threshold of realization. A large amount of clinical work has shown the very real benefits that such a method could provide. At the same time a considerable effort has been put into theoretical studies of its probable success. At present there exist gaps between these two realms. In this paper we review some general approaches to inverse problems to set the context for optical tomography, defining both the terms forward problem and inverse problem. An essential requirement is to treat the problem in a nonlinear fashion, by using an iterative method. This in turn requires a convenient method of evaluating the forward problem, and its derivatives and variance. Photon transport models are described and methods for obtaining analytical and numerical solutions for the most commonly used ones are reviewed. The inverse problem is approached by classical gradient-based solution methods. In order to develop practical implementations of these methods, we discuss the important topic of photon measurement density functions, which represent the derivative of the forward problem. We show some results that represent the most complex and realistic simulations of optical tomography yet developed. We suggest, in particular, that both time-resolved, and intensity-modulated systems can reconstruct variations in both optical absorption and scattering, but that unmodulated, non-time-resolved systems are prone to severe artefact. We believe that optical tomography reconstruction methods can now be reliably applied to a wide variety of real clinical data. The expected resolution of the method is poor, meaning that it is unlikely that the type of high-resolution images seen in computed tomography or medical resonance imaging can ever be obtained. Nevertheless we strongly expect the functional nature of these images to have a high degree of clinical significance.},
author = {Arridge, Simon R. and Schweiger, Martin},
doi = {10.1098/rstb.1997.0054},
file = {:Users/ap/Downloads/rstb.1997.0054.pdf:pdf},
issn = {09628436},
journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
number = {1354},
pages = {717--726},
title = {{Image reconstruction in optical tomography}},
volume = {352},
year = {1997}
}
@article{aggarwal2018modl,
abstract = {We introduce a model-based image reconstruction framework with a convolution neural network (CNN)-based regularization prior. The proposed formulation provides a systematic approach for deriving deep architectures for inverse problems with the arbitrary structure. Since the forward model is explicitly accounted for, a smaller network with fewer parameters is sufficient to capture the image information compared to direct inversion approaches. Thus, reducing the demand for training data and training time. Since we rely on end-to-end training with weight sharing across iterations, the CNN weights are customized to the forward model, thus offering improved performance over approaches that rely on pre-trained denoisers. Our experiments show that the decoupling of the number of iterations from the network complexity offered by this approach provides benefits, including lower demand for training data, reduced risk of overfitting, and implementations with significantly reduced memory footprint. We propose to enforce data-consistency by using numerical optimization blocks, such as conjugate gradients algorithm within the network. This approach offers faster convergence per iteration, compared to methods that rely on proximal gradients steps to enforce data consistency. Our experiments show that the faster convergence translates to improved performance, primarily when the available GPU memory restricts the number of iterations.},
archivePrefix = {arXiv},
arxivId = {1712.02862},
author = {Aggarwal, Hemant K. and Mani, Merry P. and Jacob, Mathews},
doi = {10.1109/TMI.2018.2865356},
eprint = {1712.02862},
file = {:Users/ap/Downloads/1712.02862.pdf:pdf},
issn = {1558254X},
journal = {IEEE Transactions on Medical Imaging},
keywords = {Deep learning,convolutional neural network,parallel imaging},
number = {2},
pages = {394--405},
publisher = {IEEE},
title = {{MoDL: Model-Based Deep Learning Architecture for Inverse Problems}},
volume = {38},
year = {2019}
}
@article{benning2018modern,
abstract = {Regularization methods are a key tool in the solution of inverse problems. They are used to introduce prior knowledge and allow a robust approximation of ill-posed (pseudo-) inverses. In the last two decades interest has shifted from linear to nonlinear regularization methods, even for linear inverse problems. The aim of this paper is to provide a reasonably comprehensive overview of this shift towards modern nonlinear regularization methods, including their analysis, applications and issues for future research. In particular we will discuss variational methods and techniques derived from them, since they have attracted much recent interest and link to other fields, such as image processing and compressed sensing. We further point to developments related to statistical inverse problems, multiscale decompositions and learning theory.},
archivePrefix = {arXiv},
arxivId = {1801.09922},
author = {Benning, Martin and Burger, Martin},
doi = {10.1017/S0962492918000016},
eprint = {1801.09922},
file = {:Users/ap/Library/Application Support/Mendeley Desktop/Downloaded/Benning, Burger - 2018 - Modern regularization methods for inverse problems.pdf:pdf},
issn = {14740508},
journal = {Acta Numerica},
pages = {1--111},
publisher = {Cambridge University Press},
title = {{Modern regularization methods for inverse problems}},
volume = {27},
year = {2018}
}
@article{Hammernik2018,
abstract = {Purpose: To allow fast and high-quality reconstruction of clinical accelerated multi-coil MR data by learning a variational network that combines the mathematical structure of variational models with deep learning. Theory and Methods: Generalized compressed sensing reconstruction formulated as a variational model is embedded in an unrolled gradient descent scheme. All parameters of this formulation, including the prior model defined by filter kernels and activation functions as well as the data term weights, are learned during an offline training procedure. The learned model can then be applied online to previously unseen data. Results: The variational network approach is evaluated on a clinical knee imaging protocol for different acceleration factors and sampling patterns using retrospectively and prospectively undersampled data. The variational network reconstructions outperform standard reconstruction algorithms, verified by quantitative error measures and a clinical reader study for regular sampling and acceleration factor 4. Conclusion: Variational network reconstructions preserve the natural appearance of MR images as well as pathologies that were not included in the training data set. Due to its high computational performance, that is, reconstruction time of 193 ms on a single graphics card, and the omission of parameter tuning once the network is trained, this new approach to image reconstruction can easily be integrated into clinical workflow. Magn Reson Med 79:3055–3071, 2018. {\textcopyright} 2017 International Society for Magnetic Resonance in Medicine.},
archivePrefix = {arXiv},
arxivId = {1704.00447},
author = {Hammernik, Kerstin and Klatzer, Teresa and Kobler, Erich and Recht, Michael P. and Sodickson, Daniel K. and Pock, Thomas and Knoll, Florian},
doi = {10.1002/mrm.26977},
eprint = {1704.00447},
file = {:Users/ap/Downloads/Pock{\_}VariationalNetwork{\_}MRI{\_}2017{\_}ArXiV.pdf:pdf},
issn = {15222594},
journal = {Magnetic Resonance in Medicine},
keywords = {accelerated MRI,compressed sensing,deep learning,image reconstruction,parallel imaging,variational network},
number = {6},
pages = {3055--3071},
title = {{Learning a variational network for reconstruction of accelerated MRI data}},
volume = {79},
year = {2018}
}
@inproceedings{schlemper2017deep,
author = {Schlemper, Jo and Caballero, Jose and Hajnal, Joseph V and Price, Anthony and Rueckert, Daniel},
booktitle = {International Conference on Information Processing in Medical Imaging},
file = {:Users/ap/Downloads/1703.00555.pdf:pdf},
organization = {Springer},
pages = {647--658},
title = {{A deep cascade of convolutional neural networks for MR image reconstruction}},
year = {2017}
}
@article{Kaltenbacher2011,
abstract = {Parameter identification problems for partial differential equations usually lead to nonlinear inverse problems. A typical property of such problems is their instability, which requires regularization techniques, like, e.g., Tikhonov regularization. The main focus of this paper will be on efficient methods for determining a suitable regularization parameter by using adaptive finite element discretizations based on goal-oriented error estimators. A well-established method for the determination of a regularization parameter is the discrepancy principle where the residual norm, considered as a function i of the regularization parameter, should equal an appropriate multiple of the noise level. We suggest to solve the resulting scalar nonlinear equation by an inexact Newton method, where in each iteration step, a regularized problem is solved at a different discretization level. The proposed algorithm is an extension of the method suggested in Griesbaum A et al (2008 Inverse Problems 24 025025) for linear inverse problems, where goal-oriented error estimators for i and its derivative are used for adaptive refinement strategies in order to keep the discretization level as coarse as possible to save computational effort but fine enough to guarantee global convergence of the inexact Newton method. This concept leads to a highly efficient method for determining the Tikhonov regularization parameter for nonlinear ill-posed problems. Moreover, we prove that with the so-obtained regularization parameter and an also adaptively discretized Tikhonov minimizer, usual convergence and regularization results from the continuous setting can be recovered. As a matter of fact, it is shown that it suffices to use stationary points of the Tikhonov functional. The efficiency of the proposed method is demonstrated by means of numerical experiments. {\textcopyright} 2011 IOP Publishing Ltd.},
author = {Kaltenbacher, Barbara and Kirchner, Alana and Vexler, Boris},
doi = {10.1088/0266-5611/27/12/125008},
file = {:Users/ap/Downloads/Kaltenbacher{\_}2011{\_}Inverse{\_}Problems{\_}27{\_}125008.pdf:pdf},
issn = {02665611},
journal = {Inverse Problems},
number = {12},
title = {{Adaptive discretizations for the choice of a Tikhonov regularization parameter in nonlinear inverse problems}},
volume = {27},
year = {2011}
}
@article{Adler2017,
abstract = {We propose a partially learned approach for the solution of ill-posed inverse problems with not necessarily linear forward operators. The method builds on ideas from classical regularisation theory and recent advances in deep learning to perform learning while making use of prior information about the inverse problem encoded in the forward operator, noise model and a regularising functional. The method results in a gradient-like iterative scheme, where the 'gradient' component is learned using a convolutional network that includes the gradients of the data discrepancy and regulariser as input in each iteration. We present results of such a partially learned gradient scheme on a nonlinear tomographic inversion problem with simulated data from both the Sheep-Logan phantom as well as a head CT. The outcome is compared against filtered backprojection and total variation reconstruction and the proposed method provides a 5.4 dB PSNR improvement over the total variation reconstruction while being significantly faster, giving reconstructions of 512 × 512 pixel images in about 0.4 s using a single graphics processing unit (GPU).},
archivePrefix = {arXiv},
arxivId = {1704.04058},
author = {Adler, Jonas and {\"{O}}ktem, Ozan},
doi = {10.1088/1361-6420/aa9581},
eprint = {1704.04058},
file = {:Users/ap/Downloads/Adler{\_}2017{\_}Inverse{\_}Problems{\_}33{\_}124007.pdf:pdf},
issn = {13616420},
journal = {Inverse Problems},
keywords = {deep learning,gradient descent,regularization,tomography},
number = {12},
publisher = {IOP Publishing},
title = {{Solving ill-posed inverse problems using iterative deep neural networks}},
volume = {33},
year = {2017}
}
@article{Yang2016,
abstract = {Compressive Sensing (CS) is an effective approach for fast Magnetic Resonance Imaging (MRI). It aims at reconstructing MR image from a small number of under-sampled data in k-space, and accelerating the data acquisition in MRI. To improve the current MRI system in reconstruction accuracy and computational speed, in this paper, we propose a novel deep architecture, dubbed ADMM-Net. ADMM-Net is defined over a data flow graph, which is derived from the iterative procedures in Alternating Direction Method of Multipliers (ADMM) algorithm for optimizing a CS-based MRI model. In the training phase, all parameters of the net, e.g., image transforms, shrinkage functions, etc., are discriminatively trained end-to-end using L-BFGS algorithm. In the testing phase, it has computational overhead similar to ADMM but uses optimized parameters learned from the training data for CS-based reconstruction task. Experiments on MRI image reconstruction under different sampling ratios in k-space demonstrate that it significantly improves the baseline ADMM algorithm and achieves high reconstruction accuracies with fast computational speed.},
author = {Yang, Yan and Sun, Jian and Li, Huibin and Xu, Zongben},
file = {:Users/ap/Downloads/6406-deep-admm-net-for-compressive-sensing-mri.pdf:pdf},
issn = {10495258},
journal = {Advances in Neural Information Processing Systems},
number = {Nips},
pages = {10--18},
title = {{Deep ADMM-Net for compressive sensing MRI}},
year = {2016}
}
@article{Ye2018,
abstract = {Recently, deep learning approaches with various network architectures have achieved significant performance improvement over existing iterative reconstruction methods in various imaging problems. However, it is still unclear why these deep learning architectures work for specific inverse problems. Moreover, in contrast to the usual evolution of signal processing theory around the classical theories, the link between deep learning and the classical signal processing approaches, such as wavelets, nonlocal processing, and compressed sensing, are not yet well understood. To address these issues, here we show that the long-sought missing link is the convolution framelets for representing a signal by convolving local and nonlocal bases. The convolution framelets were originally developed to generalize the theory of low-rank Hankel matrix approaches for inverse problems, and this paper further extends this idea so as to obtain a deep neural network using multilayer convolution framelets with perfect reconstruction (PR) under rectified linear unit (ReLU) nonlinearity. Our analysis also shows that the popular deep network components such as residual blocks, redundant filter channels, and concatenated ReLU (CReLU) do indeed help to achieve PR, while the pooling and unpooling layers should be augmented with high-pass branches to meet the PR condition. Moreover, by changing the number of filter channels and bias, we can control the shrinkage behaviors of the neural network. This discovery reveals the limitations of many existing deep learning architectures for inverse problems, and leads us to propose a novel theory for a deep convolutional framelet neural network. Using numerical experiments with various inverse problems, we demonstrate that our deep convolutional framelets network shows consistent improvement over existing deep architectures. This discovery suggests that the success of deep learning stems not from a magical black box, but rather from the power of a novel signal representation using a nonlocal basis combined with a data-driven local basis, which is indeed a natural extension of classical signal processing theory.},
archivePrefix = {arXiv},
arxivId = {1707.00372},
author = {Ye, Jong Chul and Han, Yoseob and Cha, Eunju},
doi = {10.1137/17M1141771},
eprint = {1707.00372},
file = {:Users/ap/Downloads/17m1141771.pdf:pdf},
issn = {19364954},
journal = {SIAM Journal on Imaging Sciences},
keywords = {Convolutional neural network,Deep learning,Framelets,Inverse problems,Perfect reconstruction condition,ReLU},
number = {2},
pages = {991--1048},
title = {{Deep convolutional framelets: A general deep learning framework for inverse problems}},
volume = {11},
year = {2018}
}
@article{Zhu2018,
abstract = {Image reconstruction is essential for imaging applications across the physical and life sciences, including optical and radar systems, magnetic resonance imaging, X-ray computed tomography, positron emission tomography, ultrasound imaging and radio astronomy. During image acquisition, the sensor encodes an intermediate representation of an object in the sensor domain, which is subsequently reconstructed into an image by an inversion of the encoding function. Image reconstruction is challenging because analytic knowledge of the exact inverse transform may not exist a priori, especially in the presence of sensor non-idealities and noise. Thus, the standard reconstruction approach involves approximating the inverse function with multiple ad hoc stages in a signal processing chain, the composition of which depends on the details of each acquisition strategy, and often requires expert parameter tuning to optimize reconstruction performance. Here we present a unified framework for image reconstruction - automated transform by manifold approximation (AUTOMAP) - which recasts image reconstruction as a data-driven supervised learning task that allows a mapping between the sensor and the image domain to emerge from an appropriate corpus of training data. We implement AUTOMAP with a deep neural network and exhibit its flexibility in learning reconstruction transforms for various magnetic resonance imaging acquisition strategies, using the same network architecture and hyperparameters. We further demonstrate that manifold learning during training results in sparse representations of domain transforms along low-dimensional data manifolds, and observe superior immunity to noise and a reduction in reconstruction artefacts compared with conventional handcrafted reconstruction methods. In addition to improving the reconstruction performance of existing acquisition methodologies, we anticipate that AUTOMAP and other learned reconstruction approaches will accelerate the development of new acquisition strategies across imaging modalities.},
archivePrefix = {arXiv},
arxivId = {1704.08841},
author = {Zhu, Bo and Liu, Jeremiah Z. and Cauley, Stephen F. and Rosen, Bruce R. and Rosen, Matthew S.},
doi = {10.1038/nature25988},
eprint = {1704.08841},
file = {:Users/ap/Downloads/nature25988.pdf:pdf},
issn = {14764687},
journal = {Nature},
number = {7697},
pages = {487--492},
publisher = {Nature Publishing Group},
title = {{Image reconstruction by domain-transform manifold learning}},
volume = {555},
year = {2018}
}
@article{hammernik2018learning,
author = {Hammernik, Kerstin and Klatzer, Teresa and Kobler, Erich and Recht, Michael P and Sodickson, Daniel K and Pock, Thomas and Knoll, Florian},
file = {:Users/ap/Downloads/mrm.26977.pdf:pdf},
journal = {Magnetic resonance in medicine},
number = {6},
pages = {3055--3071},
publisher = {Wiley Online Library},
title = {{Learning a variational network for reconstruction of accelerated MRI data}},
volume = {79},
year = {2018}
}
@article{chen2017low,
author = {Chen, Hu and Zhang, Yi and Kalra, Mannudeep K and Lin, Feng and Chen, Yang and Liao, Peixi and Zhou, Jiliu and Wang, Ge},
file = {:Users/ap/Downloads/07947200.pdf:pdf},
journal = {IEEE transactions on medical imaging},
keywords = {Denoiser},
mendeley-tags = {Denoiser},
number = {12},
pages = {2524--2535},
publisher = {IEEE},
title = {{Low-dose CT with a residual encoder-decoder convolutional neural network}},
volume = {36},
year = {2017}
}
@article{kang2017deep,
author = {Kang, Eunhee and Min, Junhong and Ye, Jong Chul},
file = {:Users/ap/Downloads/mp.12344.pdf:pdf},
journal = {Medical physics},
keywords = {Denoiser},
mendeley-tags = {Denoiser},
number = {10},
pages = {e360----e375},
publisher = {Wiley Online Library},
title = {{A deep convolutional neural network using directional wavelets for low-dose X-ray CT reconstruction}},
volume = {44},
year = {2017}
}
@article{Gupta2018,
abstract = {We present a new image reconstruction method that replaces the projector in a projected gradient descent (PGD) with a convolutional neural network (CNN). Recently, CNNs trained as image-to-image regressors have been successfully used to solve inverse problems in imaging. However, unlike existing iterative image reconstruction algorithms, these CNN-based approaches usually lack a feedback mechanism to enforce that the reconstructed image is consistent with the measurements. We propose a relaxed version of PGD wherein gradient descent enforces measurement consistency, while a CNN recursively projects the solution closer to the space of desired reconstruction images. We show that this algorithm is guaranteed to converge and, under certain conditions, converges to a local minimum of a non-convex inverse problem. Finally, we propose a simple scheme to train the CNN to act like a projector. Our experiments on sparse-view computed-tomography reconstruction show an improvement over total variation-based regularization, dictionary learning, and a state-of-the-art deep learning-based direct reconstruction technique.},
archivePrefix = {arXiv},
arxivId = {1709.01809},
author = {Gupta, Harshit and Jin, Kyong Hwan and Nguyen, Ha Q. and McCann, Michael T. and Unser, Michael},
doi = {10.1109/TMI.2018.2832656},
eprint = {1709.01809},
file = {:Users/ap/Downloads/08353870.pdf:pdf},
issn = {1558254X},
journal = {IEEE Transactions on Medical Imaging},
keywords = {Deep learning,biomedical image reconstruction,inverse problems,low-dose computed tomography},
number = {6},
pages = {1440--1453},
publisher = {IEEE},
title = {{CNN-Based Projected Gradient Descent for Consistent CT Image Reconstruction}},
volume = {37},
year = {2018}
}
@article{Zhang2017,
author = {Zhang, Lei and Zuo, Wangmeng},
file = {:Users/ap/Downloads/08026108.pdf:pdf},
journal = {IEEE Signal Processing Magazine},
number = {September},
title = {{Image restoration: From sparse and low-rank priors to deep priors}},
year = {2017}
}
@article{Antun2019,
abstract = {Deep learning, due to its unprecedented success in tasks such as image classification, has emerged as a new tool in image reconstruction with potential to change the field. In this paper we demonstrate a crucial phenomenon: deep learning typically yields unstablemethods for image reconstruction. The instabilities usually occur in several forms: (1) tiny, almost undetectable perturbations, both in the image and sampling domain, may result in severe artefacts in the reconstruction, (2) a small structural change, for example a tumour, may not be captured in the reconstructed image and (3) (a counterintuitive type of instability) more samples may yield poorer performance. Our new stability test with algorithms and easy to use software detects the instability phenomena. The test is aimed at researchers to test their networks for instabilities and for government agencies, such as the Food and Drug Administration (FDA), to secure safe use of deep learning methods.},
archivePrefix = {arXiv},
arxivId = {1902.05300},
author = {Antun, Vegard and Renna, Francesco and Poon, Clarice and Adcock, Ben and Hansen, Anders C.},
eprint = {1902.05300},
file = {:Users/ap/Downloads/1902.05300.pdf:pdf},
title = {{On instabilities of deep learning in image reconstruction - Does AI come at a cost?}},
url = {http://arxiv.org/abs/1902.05300},
year = {2019}
}
@article{McCann2017,
abstract = {In this article, we review recent uses of convolutional neural networks (CNNs) to solve inverse problems in imaging. It has recently become feasible to train deep CNNs on large databases of images, and they have shown outstanding performance on object classification and segmentation tasks. Motivated by these successes, researchers have begun to apply CNNs to the resolution of inverse problems such as denoising, deconvolution, superresolution, and medical image reconstruction, and they have started to report improvements over state-of-the-art methods, including sparsity-based techniques such as compressed sensing. Here, we review the recent experimental work in these areas, with a focus on the critical design decisions.},
archivePrefix = {arXiv},
arxivId = {1710.04011},
author = {McCann, Michael T. and Jin, Kyong Hwan and Unser, Michael},
doi = {10.1109/MSP.2017.2739299},
eprint = {1710.04011},
file = {:Users/ap/Downloads/McCannUnser{\_}review2017.pdf:pdf},
issn = {10535888},
journal = {IEEE Signal Processing Magazine},
number = {6},
pages = {85--95},
title = {{Convolutional neural networks for inverse problems in imaging: A review}},
volume = {34},
year = {2017}
}
@article{Espeholt2018,
abstract = {In this work we aim to solve a large collection of tasks using a single reinforcement learning agent with a single set of parameters. A key challenge is to handle the increased amount of data and ex- ; tended training time. We have developed a new distributed agent IMPALA (Importance Weighted Actor-Learner Architecture) that not only uses j resources more efficiently in single-machine train- ' ing but also scales to thousands of machines with- ; out sacrificing data efficiency or resource utilisation. We achieve stable learning at high through- ' put by combining decoupled acting and learning with a novel off-policy correction method called V-trace. We demonstrate the effectiveness of IMPALA for multi-task reinforcement learning on • DMLab-30 (a set of 30 tasks from the DeepMind Lab environment (Beattie et al., 2016)) and Atari- 57 (all available Atari games in Arcade Learning Environment (Bellemare et al., 2013a)). Our results show that IMPALA is able to achieve better ; performance than previous agents with less data, and crucially exhibits positive transfer between tasks as a result of its multi-task approach.},
archivePrefix = {arXiv},
arxivId = {1802.01561},
author = {Espeholt, Lasse and Soyer, Hubert and Munos, Remi and Simonyan, Karen and Mnih, Volodymyr and Ward, Tom and Yotam, Boron and Vlad, Firoiu and Tim, Harley and Dunning, Iain and Legg, Shane and Kavukcuoglu, Koray},
eprint = {1802.01561},
file = {:Users/ap/Downloads/1802.01561.pdf:pdf},
isbn = {9781510867963},
journal = {35th International Conference on Machine Learning, ICML 2018},
pages = {2263--2284},
title = {{IMPALA: Scalable Distributed Deep-RL with Importance Weighted Actor-Learner Architectures}},
volume = {4},
year = {2018}
}
@inproceedings{rick2017one,
author = {{Rick Chang}, J H and Li, Chun-Liang and Poczos, Barnabas and {Vijaya Kumar}, B V K and Sankaranarayanan, Aswin C},
booktitle = {Proceedings of the IEEE International Conference on Computer Vision},
file = {:Users/ap/Downloads/Chang{\_}One{\_}Network{\_}to{\_}ICCV{\_}2017{\_}paper.pdf:pdf},
pages = {5888--5897},
title = {{One Network to Solve Them All--Solving Linear Inverse Problems Using Deep Projection Models}},
year = {2017}
}
@article{Dong2017,
abstract = {In the past few decades, mathematics based approaches have been widely adopted in various image restoration problems; the partial differential equation (PDE) based approach (e.g., the total variation model [L. Rudin, S. Osher, and E. Fatemi, Phys. D, 60 (1992), pp. 259-268] and its generalizations, nonlinear diffusions [P. Perona and J. Malik, IEEE Trans. Pattern Anal. Mach. Intel., 12 (1990), pp. 629-639; F. Catte et al., SIAM J. Numer. Anal., 29 (1992), pp. 182-193], etc.) and wavelet frame based approach are some successful examples. These approaches were developed through different paths and generally provided understanding from different angles of the same problem. As shown in numerical simulations, implementations of the wavelet frame based approach and the PDE based approach quite often end up solving a similar numerical problem with similar numerical behaviors, even though different approaches have advantages in different applications. Since wavelet frame based and PDE based approaches have all been modeling the same types of problems with success, it is natural to ask whether the wavelet frame based approach is fundamentally connected with the PDE based approach when we trace them all the way back to their roots. A fundamental connection of a wavelet frame based approach with a total variation model and its generalizations was established in [J. Cai, B. Dong, S. Osher, and Z. Shen, J. Amer. Math. Soc., 25 (2012), pp. 1033-1089]. This connection gives the wavelet frame based approach a geometric explanation and, at the same time, it equips a PDE based approach with a time frequency analysis. Cai et al. showed that a special type of wavelet frame model using generic wavelet frame systems can be regarded as an approximation of a generic variational model (with the total variation model as a special case) in the discrete setting. A systematic convergence analysis, as the resolution of the image goes to infinity, which is the key step in linking the two approaches, is also given in Cai et al. Motivated by Cai et al. and [Q. Jiang, Appl. Numer. Math., 62 (2012), pp. 51-66], this paper establishes a fundamental connection between the wavelet frame based approach and nonlinear evolution PDEs, provides interpretations and analytical studies of such connections, and proposes new algorithms for image restoration based on the new understandings. Together with the results in [J. Cai et al., J. Amer. Math. Soc., 25 (2012), pp. 1033-1089], we now have a better picture of how the wavelet frame based approach can be used to interpret the general PDE based approach (e.g., the variational models or nonlinear evolution PDEs) and can be used as a new and useful tool in numerical analysis to discretize and solve various variational and PDE models. To be more precise, we shall establish the following: (1) The connections between wavelet frame shrinkage and nonlinear evolution PDEs provide new and inspiring interpretations of both approaches that enable us to derive new PDE models and (better) wavelet frame shrinkage algorithms for image restoration. (2) A generic nonlinear evolution PDE (of parabolic or hyperbolic type) can be approximated by wavelet frame shrinkage with properly chosen wavelet frame systems and carefully designed shrinkage functions. (3) The main idea of this work is beyond the scope of image restoration. Our analysis and discussions indicate that wavelet frame shrinkage is a new way of solving PDEs in general, which will provide a new insight that will enrich the existing theory and applications of numerical PDEs, as well as those of wavelet frames.},
author = {Dong, Bin and Jiang, Qingtang and Shen, Zuowei},
doi = {10.1137/15M1037457},
issn = {15403467},
journal = {Multiscale Modeling and Simulation},
keywords = {Image restoration,Nonlinear diffusion,Wavelet frame shrinkage,Wavelet frames},
number = {1},
pages = {606--660},
title = {{Image restoration: Wavelet frame shrinkage, nonlinear evolution PDEs, and beyond}},
volume = {15},
year = {2017}
}
